Do LLMs Find Human Answers To Fact-Driven Questions Perplexing? A Case Study on Reddit

Large language models (LLMs) have been shown to be proficient in correctly answering questions in the context of online discourse. However, the study of using LLMs to model human-like answers to fact-driven social media questions is still under-explored. In this work, we investigate how LLMs model the wide variety of human answers to fact-driven questions posed on several topic-specific Reddit communities, or subreddits. We collect and release a dataset of 409 fact-driven questions and 7,534 diverse, human-rated answers from 15 r/Ask{Topic} communities across 3 categories: profession, social identity, and geographic location. We find that LLMs are considerably better at modeling highly-rated human answers to such questions, as opposed to poorly-rated human answers. We present several directions for future research based on our initial findings.

==> sections/conclusion.tex <==
\section{Conclusion}

In this study, we explore the capacity of large pre-trained language models (LLMs) to capture a diverse range of human answers to factual questions asked in various r/Ask{Topic} online communities. We filter and make available a dataset containing 409 factual questions and 7,534 answers with diverse ratings from 15 r/Ask{Topic} communities spanning three topic categories: profession, social identity, and geographic location. Our analysis reveals that LLMs excel at modeling well-rated human responses to these questions compared to lower-rated responses. We propose several promising avenues for future research based on these preliminary results.
